SpectAcLE: An Improved Method for Modeling Light Echo Spectra

Light echoes give us a unique perspective on the nature of supernovae and non-terminal stellar explosions. Spectroscopy of light echoes can reveal details on the kinematics of the ejecta, probe asymmetry, and reveal details on its interaction with circumstellar matter, thus expanding our understanding of these transient events. However, the spectral features arise from a complex interplay between the source photons, the reflecting dust geometry, and the instrumental setup and observing conditions. In this work we present an improved method for modeling these effects in light echo spectra, one that relaxes the simplifying assumption of a light curve weighted sum, and instead estimates the true relative contribution of each phase. We discuss our logic, the gains we obtain over light echo analysis method(s) used in the past, and prospects for further improvements. Lastly, we show how the new method improves our analysis of echoes from Tycho's supernova (SN 1572) as an example.

==> 02Appendices/04Effective_PSF.tex <==
\section{Effective PSF}
\label{sec:eff_PSF}
\noindent {\bf Effective PSF:} In general, the PSF of an observation is measured in terms of the Full-Width-Half-Maximum (FWHM). For our purposes, the PSF usually can be sufficiently characterized with a circular Gaussian having a single width $\sigma_{\rm PSF}$, as measured by standard PSF photometry.
% The $\sigma_{PSF}$ of that Gaussian can be calculated as \redpen{FILL ME: equation}. % RP: what do you mean calculate sigma_PSF? It's measured by photometry on the image
We denote the angle between the the light echo profile box $A_{\rm box}$ and the line perpendicular to the ``crest'' of the light echo $A_{\rm LE}$ (maximum projection scale) as $\alpha$, such that $\alpha=0$ when the profile box is perpendicular to the crest ($A_{0,{\rm box}}=A_{\rm LE}$). Then $\sigma_{\rm PSF,eff}$ is related to $\sigma_{\rm PSF}$ with the following relation:

\begin{eqnarray}
\sigma_{\rm PSF,eff}  =  \frac{\sigma_{\rm PSF}}{\cos{\alpha}} \label{eq:PSF_eff}
\end{eqnarray}
 
We note that for small angles of $\alpha$, $\sigma_{\rm PSF,eff} \approx \sigma_{\rm PSF}$. This is not a big effect, and needs to be taken into account only for $\alpha\gtrsim15\deg$ (see Figure~\ref{fig:eff_psf}).
This means that for cases with large $\alpha$, we must estimate the position angle of the ellipsoid-dust intersection arclet $A_{\rm LE}$ in order to get $\sigma_{\rm PSF,eff}$ (see step 2 in Section~\ref{sec:mthd_proc}).
\\\\

\begin{figure}
\epsscale{1.0}
\includegraphics[width=\linewidth]{figures/07_Appendices/effective_psf_v2.png}
\figcaption{Effect of position angle on effective PSF. For a given PSF (in this case a circular one for simplicity), it's effective width on the light echo profile will be wider for shallower angles in respect to $A_{LE}$ (see \ref{fig:prinicipalaxes}). \label{fig:eff_psf}}
\end{figure}

